Meta 3D TextureGen: Fast and Consistent Texture Generation for 3D Objects

The recent availability and adaptability of text-to-image models has sparked a new era in many related domains that benefit from the learned text priors as well as high-quality and fast generation capabilities, one of which is texture generation for 3D objects. Although recent texture generation methods achieve impressive results by using text-to-image networks, the combination of global consistency, quality, and speed, which is crucial for advancing texture generation to real-world applications, remains elusive. To that end, we introduce Meta 3D TextureGen: a new feedforward method comprised of two sequential networks aimed at generating high-quality and globally consistent textures for arbitrary geometries of any complexity degree in less than 20 seconds. Our method achieves state-of-the-art results in quality and speed by conditioning a text-to-image model on 3D semantics in 2D space and fusing them into a complete and high-resolution UV texture map, as demonstrated by extensive qualitative and quantitative evaluations. In addition, we introduce a texture enhancement network that is capable of up-scaling any texture by an arbitrary ratio, producing 4k pixel resolution textures.

==> figures/data_figure/fig_data.tex <==
\begin{figure}[t]
\centering

\begin{minipage}{\linewidth}
	\centering

    % Position
    \fbox{
    \begin{minipage}{0.22\linewidth}
	    \centering
        \includegraphics[width=0.45\linewidth]{figures/data_figure/position_000.jpg}
        \includegraphics[width=0.45\linewidth]{figures/data_figure/position_001.jpg}
        \includegraphics[width=0.45\linewidth]{figures/data_figure/position_002.jpg}
        \includegraphics[width=0.45\linewidth]{figures/data_figure/position_003.jpg}
	    %(a)
	\end{minipage}
    }
    \begin{minipage}{0.22\linewidth}
	    \centering
        \includegraphics[width=\linewidth]{figures/data_figure/position_uv.jpg}
	    %(a)
	\end{minipage}
    \fbox{
    \begin{minipage}{0.22\linewidth}
	    \centering
        \includegraphics[width=0.45\linewidth]{figures/data_figure/normal_000.jpg}
        \includegraphics[width=0.45\linewidth]{figures/data_figure/normal_001.jpg}
        \includegraphics[width=0.45\linewidth]{figures/data_figure/normal_002.jpg}
        \includegraphics[width=0.45\linewidth]{figures/data_figure/normal_003.jpg}
	    %(a)
	\end{minipage}
    }
    \begin{minipage}{0.22\linewidth}
	    \centering
        \includegraphics[width=\linewidth]{figures/data_figure/normal_uv.jpg}
	    %(a)
	\end{minipage}

    % \Large{\emph{``a realistic armadillo creature with a \textbf{\textcolor{turtlegreen}{shell like a green turtle}} on its back''}}

\end{minipage}

	%\begin{tabular}{@{}c@{\,}c@{\,}c@{}}
%
		%\includegraphics[width=0.33\linewidth]{images/mesh040_mesh018} &
		%\includegraphics[width=0.33\linewidth]{images/david11_david13_10} &
		%\includegraphics[width=0.33\linewidth]{images/michael2_victoria23} \\
		%
		%(a) & (b) & (c) \\
		%
		%\includegraphics[width=0.33\linewidth]{images/michael4_gorilla14_7} &
		%\includegraphics[width=0.33\linewidth]{images/cat3_cat2} &
		%\includegraphics[width=0.33\linewidth]{images/centaur3_centaur0_7} \\
%
		%(d) & (e) & (f) \\
%
	%\end{tabular}

\caption{Position and normal renders (left) and UV maps (right) used as conditioning. \emph{First row}: Position renders. \emph{Second row}: Normal renders.}
\label{fig:position_normal}
% \vspace{-5mm}
\end{figure}

